Visualization techniques for the developing chicken heart

We present a geometric surface parameterization algorithm and several visualization techniques adapted to the problem of understanding the 4D peristaltic-like motion of the outflow tract (OFT) in an embryonic chick heart. We illustrated the techniques using data from hearts under normal conditions (four embryos), and hearts in which blood flow conditions are altered through OFT banding (four embryos). The overall goal is to create quantitative measures of the temporal heart-shape change both within a single subject and between multiple subjects. These measures will help elucidate how altering hemodynamic conditions changes the shape and motion of the OFT walls, which in turn influence the stresses and strains on the developing heart, causing it to develop differently. We take advantage of the tubular shape and periodic motion of the OFT to produce successively lower dimensional visualizations of the cardiac motion (e.g. curvature, volume, and cross-section) over time, and quantifications of such visualizations.

==> todo.tex <==
TOODOS

Introduction
\begin{itemize}
\item Need cross section contours for opening and closing
\end{itemize}

%Related work
%\begin{itemize}
%\end{itemize}

Data
\begin{itemize}
\item Sandra: Check control group is normal or sham embryos
\item Sandra - which ref do you want on page 9 4D image sets were then segmented....
\end{itemize}

Parameterization
\begin{itemize}
\item Just a note in general - I'm using one of Ly's figures from her thesis which is the new algorithm (fig:param). It's qualitatively correct, so I think that's ok. Similarly, I'm fudging a bit on the temporal smoothing of the end points. We could just take it out, but...
\end{itemize}

Contract
\begin{itemize}
\item I redid the quiver plot; should probably do with arrows, but need Ly's original data to do this.
\end{itemize}

Shape
\begin{itemize}
\item Ly: Redo strain images with a better color map
\end{itemize}

Results
\begin{itemize}
\item Re-do table with actual times for slopes
\item Change plot y axes labels figure 13
\end{itemize}

Supplemental
\begin{itemize}
\item Volume plots for each chick [missing 4th and 8th chick]
\item Cross section area complete plot
\item Cross section versus time area plots for all three surfaces
\end{itemize}
